Exploring D3 Implementation Challenges on Stack Overflow

Visualization languages help to standardize the process of designing effective visualizations, one of the most prominent being D3. However, few researchers have analyzed at scale how users incorporate these languages into existing visualization programming processes, i.e., implementation workflows. In this paper, we present an analysis of the experiences of D3 users as observed through Stack Overflow, summarizing common D3 implementation workflows and challenges discussed online. Our results show how the visualization community may be limiting its understanding of users' visualization implementation challenges by ignoring the larger context in which languages such as D3 are used. Based on our findings, we suggest new research directions to enhance the user experience with visualization languages. All our data and code are available at: https://osf.io/fup48/.

==> content/acknowledgements.tex <==
\section{Acknowledgements}
We thank all the reviewers, study participants, and members of both the Human-Computer Interaction Lab and the Battle Data Lab for their valuable feedback. 

==> content/conclusion.tex <==
\section{Conclusion}
\label{sec:conclusion}


==> content/usability.tex <==
\vspace{-1mm}
\section{Design Breadth: Challenges in Harnessing the Expressiveness of D3}
\label{sec:usability}
\vspace{-1.5mm}

Visualization languages are frequently evaluated by their expressiveness, in other words by the breadth and depth of the visualization and interaction design spaces that they represent~\cite{bostock_d3_2011,mei2018design,satyanarayan_vega-lite:_2017}.
However, theoretical expressiveness rarely matches what the average user does in practice.
%We observe that D3 is as much a visualization community as it is a visualization language, where the strength of communication across the community impacts the \emph{usability} of D3.
%For example, D3 is a complicated language that can be difficult to learn, yet it remains popular at least in part because of the ample documentation and support provided by the D3 community.
%We observe three overlapping groups within this community: the developer(s) maintaining D3; the researchers studying, enhancing, and/or competing with D3; and the D3 users.
In this section, we seek to understand the scope of this gap between theory and practice for D3, and how we might work towards closing it.
%
%In this section, we explore the \emph{usability} of D3 by exploring how these three groups interact (or not).
%In this case, usability is not just about how easy D3 is to use on its own, but also how easy it is for D3 users to access critical information and community support for applying visualization best practices through D3.
For example, to understand whether the expressiveness of D3 has translated to many novel visualizations from Stack Overflow users, we can compare the frequency and breadth of visualization types observed for D3 on Stack Overflow and in the academic literature.
If we observe a significant gap between what D3 enables and what users actually do, we can investigate potential causes by analyzing D3's support infrastructure, such as by analyzing how these different visualization types are supported by existing examples and the D3 documentation.  We can perform a similar analysis for interaction types.
%We can also analyze how D3 users utilize different interaction types from the academic literature by analyzing the frequency and breadth of interactions discussed.
%In this way, we can note limitations in the usability of D3 through communication barriers, such as skewed preferences for visualization and interactions, which could indicate design bias among particular groups.
We focus on two questions in this analysis regarding visualization and interaction design breadth:
\begin{itemize}[nosep]
\item \textbf{Q5}: What are D3 users' visualization preferences and how do they relate to implementation challenges in D3?
\item \textbf{Q6}: What are D3 users' interaction preferences and how do they relate to implementation challenges in D3?
\end{itemize}
%We explore these questions in two directions: the breadth of visualizations observed on Stack Overflow compared to the D3 documentation and the academic literature,
%and the breath of interactions compared to the documentation and the literature.

\begin{figure}
\centering
\includegraphics[width=0.5\columnwidth]{figures/all_vistypes.pdf}
\vspace{-5mm}
\caption{
Total observations for the top 16 visualization types observed in (a) the D3 gallery, (b) our randomized sample of qualitatively coded Stack Overflow posts, and (c) GitHub issues for D3. The top eight visualizations from the coded sample are colored blue.}
\label{fig:all-vis-types}
\vspace{-6mm}
\end{figure}

%\begin{figure}
%\centering
%\includegraphics[width=0.7\columnwidth]{figures/visualizationTypes.pdf}
%\vspace{-5mm}
%\caption{
%A bar chart showing on the y axis the total Stack Overflow posts that mention the given visualization type from our coded dataset.}
%\label{fig:vis-types}
%\vspace{-6mm}
%\end{figure}

\vspace{-1.5mm}
\subsection{Analyzing Observed Visualization Breadth}
\label{sec:usability:visualization-breadth-overview}
\vspace{-1.5mm}


%\begin{figure*}
%  \begin{subfigure}[b]{0.49\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figures/visualizationTypes_issues.pdf}
%    \caption{Visualization types Observed in the D3 GitHub Issues.}
%    \label{fig:vis-github-issues}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.47\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figures/d3-gallery.pdf}
%    \caption{Visualization Types Observed in the D3 Gallery Visual Index.}
%    \label{fig:d3-gallery}
%  \end{subfigure}
%  \vspace{-4mm}
%  \caption{Two bar charts showing on the y axis the total observed posts that mention specific visualization types from our extended visualization taxonomy, colored by popularity on Stack Overflow, either from GitHub (a) or the D3 Gallery (b).
%  }
%  \vspace{-6mm}
%\end{figure*}

\subsubsection{Analysis Method.}
We focus our analysis of visualization breadth on visualization types.
%, such as bar charts, scatterplots, or geographic maps.
Our goal is to understand how existing taxonomies compare with the breadth of visualizations discussed on Stack Overflow.
We define visualization breadth as the total distinct visualization types observed, which we base on existing evaluations of visualization and interaction design coverage (e.g., \cite{satyanarayan_vega-lite:_2017}). We use the visualization taxonomy observed by Battle et al.~\cite{battle_beagle:_2018} as our starting point, because it is based on visualizations shared by users of D3, as well as other tools such as Plotly and Fusion Charts. Battle et al. observed 24 visualization types:
\texttt{area, bar, box, bubble, chord, contour, donut, filled-line
geographic map, graph/tree, heatmap, hexabin, line, radial/radar, pie,
sankey, scatter, treemap, voronoi, waffle, word cloud,
sunburst, stream graph}, and \texttt{parallel coordinates.}
We extended this taxonomy with nine more visualization types observed on Stack Overflow (\texttt{bullet, funnel, hive, marimekko, OHLC, polygon, table, gantt}, and \texttt{waterfall}), and three more types from the D3 gallery visual index (\texttt{dial, icicle}, and \texttt{horizon}). The final taxonomy includes $24+8+4=36$ visualization types.

To analyze visualization breadth, we labeled Stack Overflow posts with any mentioned visualization types from our extended taxonomy. For example, when a user mentions bar charts: ``I'm working on creating a stacked bar chart...'' (post A-207) , we label the post with ``vis-bar''. Then, we tabulate the visualization and interaction types observed for Stack Overflow, existing taxonomies, the D3 gallery and documentation, and GitHub issues reported for D3. Finally, we compare the visualization and interaction types observed, and discuss the significance of observed differences.


%\footnote{\raggedright\url{https://stackoverflow.com/questions/46961747/dc-js-ordinal-stacked-barchart-with-two-dimensions-getting-nan-values-and-no-st}}

\vspace{-1.5mm}
\subsubsection{Stack Overflow Users Favor A Handful of Visualization Types.}
Most posts focus on a specific visualization type.
%that the user wants to implement or enhance.
We find that 48.7\% of our coded posts mention explicit visualization types; the top 16 are shown in \autoref{fig:all-vis-types} (center).
29 of the 36 visualization types from our extended taxonomy were observed (or 80.6\%), however 12 appear only once (or 33.3\%). One might assume that the most common visualization types (e.g., \texttt{bar} charts and \texttt{line} charts) are least likely to cause problems for Stack Overflow users, given their pervasiveness and simplicity.
However, the top three visualizations we observed were \texttt{bar} charts, \texttt{line} charts, and geographic \texttt{map}s, which are also three of the most common visualization types observed by Battle et al.~\cite{battle_beagle:_2018}.
More complex visualizations, such as \texttt{parallel coordinates}, are rarely mentioned in comparison. These results suggest that observed visualization types on Stack Overflow are indicative of user visualization preferences rather than complexity or challenge in implementing specific visualization types.

\vspace{-1.5mm}
\subsection{Q5: Stack Overflow Users May be Exhibiting Design Bias in Preferences for Visualization Types}
\label{sec:usability:visualization-breadth}
\vspace{-1.5mm}

\subsubsection{Complexity Does not Drive User Interest on Stack Overflow.}
However, choosing a visualization type is one of many decisions in the visualization implementation process.
We also investigated whether the mention of simpler visualization types may be due to
complexity elsewhere in the visualization, such as from implementing interactions, e.g., ``... when I change the zoom the SVG also change the location'' (post A-374). Here, we focus on \texttt{bar} charts as a case study.
We found that only 20.7\% of bar chart-related posts discuss interactions, and only 17.0\% of these posts were made by self-professed D3 newbies (34.1\% total).
Thus, we cannot we fully explain the skew towards basic visualization types on Stack Overflow simply by pointing to novices, nor to more advanced functionality elsewhere in users' visualizations. Stack Overflow users seem to prefer simpler visualization types, regardless of their programming and D3 expertise.

%\footnote{\raggedright\url{https://stackoverflow.com/questions/46961747/dc-js-ordinal-stacked-barchart-with-two-dimensions-getting-nan-values-and-no-st}}
%\footnote{\raggetright\url{https://stackoverflow.com/questions/23232929/looping-transition-in-d3}}
%\footnote{\raggedright\url{https://stackoverflow.com/questions/10883523/d3-how-to-change-the-width-and-length-of-svg}}

Despite their complexity, \texttt{tree}s and \texttt{graph}s combined are the second most frequently mentioned visualization type on Stack Overflow. This result contrasts with prior work, where \texttt{graphs/trees} do not even appear in the top five visualization types observed for D3 or other common visualization tools~\cite{battle_beagle:_2018}. Thus complexity does not seem to be a driver for which visualization types are discussed on Stack Overflow.

\vspace{-1.5mm}
\subsubsection{Stack Overflow and GitHub Users Focus on Somewhat Different Visualization Types}
We compare our findings with reported \textbf{GitHub} issues for D3 to observe how they translate across user groups. Using the search bar on the D3 GitHub issues page, we searched for mentions of each visualization type in our extended taxonomy. The results are shown in \autoref{fig:all-vis-types} (right).
%The x axis encodes visualization type, bar height the total relevant GitHub issues, and bar color the popularity of this visualization type in our coded Stack Overflow data.
31 out of 36 visualization types were observed in the GitHub issues (or 86\%). Some of the top visualization types observed in our coded dataset are also observed in the GitHub issues.
A couple of visualization types are consistent between Stack Overflow and GitHub users. For example, the popularity of \texttt{graph}s/\texttt{tree}s is similar to our results for our coded dataset, and the prevalence of \texttt{map}s is similar to the findings of Battle et al~\cite{battle_beagle:_2018}.
However, in general observations on GitHub do not match our coded dataset. For example, \texttt{bubble} and \texttt{scatterplot} visualizations are the ninth and thirteenth most common visualization types on GitHub, rather than the fifth and sixth most common as seen on Stack Overflow. Furthermore, more specialized types such as \texttt{chord} visualizations are mentioned more frequently on GitHub.
Thus, the experiences of Stack Overflow users are similar to, but may not necessarily match the implementation challenges encountered by users posting GitHub issues for D3.

\vspace{-1.5mm}
\subsubsection{Observed Visualizations on Stack Overflow Match the D3 Gallery.} We then compared the occurrence of visualization types in our coded dataset to those in the \textbf{D3 example gallery}. We labeled each visualization observed in the D3 gallery visual index using our extended taxonomy; the results are shown in \autoref{fig:all-vis-types} (left).
30 of 36 visualization types were observed in the D3 gallery visual index (or 83\%).
Similar to our findings on GitHub, \texttt{graph}s (and \texttt{tree}s) are the most popular visualization type in D3 gallery visual index, along with \texttt{map}s, \texttt{bar} charts, and \texttt{line} charts.

When we combine our findings across GitHub issues, the D3 gallery, and in previous work~\cite{battle_beagle:_2018}, our results paint a more holistic picture of users' design choices.
We see that \texttt{line} and \texttt{bar} visualizations dominate because they are universally popular across visualization tools, as shown in the work of Battle et al.~\cite{battle_beagle:_2018}. \texttt{graph} and \texttt{tree} visualizations may be of interest to Stack Overflow users because they appear frequently in the D3 gallery, documentation, and GitHub issues.
These results further support the idea that D3 users seem to rely heavily on existing D3 examples and documentation when implementing new visualizations. Thus the D3 gallery likely represents, and perhaps even influences, the range of visualizations created by Stack Overflow users. There seems to be an interesting cycle of dependence established between D3 users and developers through the documentation and through GitHub in general.

To gauge the importance of the D3 example gallery within the documentation, we analyzed how often the gallery page was updated on GitHub compared to other pages, e.g., the home
~\cite{d3home} or API reference~\cite{d3api} pages.
At the time of our analysis, the D3 Gallery page had been updated 1,295 times, three times as often as any other main page in the D3 documentation. We also found 29 GitHub issues that cited the D3 gallery visual index, supporting our findings.

\vspace{-1.5mm}
\subsection{Takeaways for Visualization Breadth Analysis}
\vspace{-1.5mm}

In response to \textbf{Q5}, Stack Overflow users seem to favor a few simple visualization types, but existing observation-based taxonomies cannot fully explain our results~\cite{battle_beagle:_2018}. For example \texttt{graph} and \texttt{tree} visualizations are discussed more on Stack Overflow than they are seen shared online~\cite{battle_beagle:_2018}, but their popularity on Stack Overflow is consistent with the prevalence of \texttt{graph} and \texttt{tree} visualizations in the D3 gallery.
These findings suggest a strong connection between Stack Overflow users and the D3 developers, captured through the D3 documentation.
However, these findings suggest that if the D3 documentation is skewed to prioritize specific visualizations, it could potentially introduce bias in to users' implementation workflows.

Given the breadth of visualization types observed in the academic literature, one interesting question for the future is why Stack Overflow users do not seem to experiment with these other visualization types. On the one hand, these findings might suggest that the full design breadth of D3 may be interesting but also overkill for most Stack Overflow users. On the other hand, given that Stack Overflow users frequently reference existing D3 visualizations as part of their implementation workflows, the issue could be that there is insufficient scaffolding for users to feel confident in creating these other types of visualizations. The quantity and variety of gallery examples may be just as important as the quality of examples in helping users expand their design thinking. We explore these ideas further in the next section.

\begin{figure}
  \centering
  \includegraphics[width=0.3\columnwidth]{figures/interactionTypes.pdf}
  \vspace{-4mm}
  \caption{Total observations (y axis) for all interaction types from our taxonomy (x axis) in the qualitatively coded Stack Overflow data.}
  \label{fig:interaction-types}
  \vspace{-6mm}
\end{figure}

\vspace{-1.5mm}
\subsection{Analyzing Observed Interaction Breadth}
\label{sec:usability:interaction-breadth-overview}
\vspace{-1.5mm}

%In this section, we dive deeper into users' engagement with the D3 documentation and academic best practices, specifically for interaction design.
\subsubsection{Analysis Methods.} In this section, we dive deeper into users' design preferences, specifically for interaction types.
We define interaction breadth as the total distinct interaction types observed, such as selection, filtering, or navigation. We use the typology proposed by Brehmer and Munzner~\cite{brehmer2013multi} for our analysis. We focus on the ``manipulate'' interactions in the typology, which summarize and align closely with other interaction taxonomies for information visualization (e.g., \cite{yi2007toward}). Brehmer and Munzner define six ``manipulate'' interactions and a separate ``encode'' interaction, which we use in our analysis:
\begin{itemize}[nosep]
\item \texttt{encode}: change the encodings
\item \texttt{select}: hover, click, lasso, or otherwise highlight marks
\item \texttt{navigate}: pan, zoom, rotate
\item \texttt{arrange}: reorder axes, change spatial layout
\item \texttt{change}: alter/format the visualization (not the encodings)
\item \texttt{filter}: include/exclude data records
\item \texttt{aggregate}: group, adjust granularity.
\end{itemize}
We stress however that this is only a subset of the ``how'' level of the Brehmer and Munzner typology, and expert D3 implementationers likely implement the full range of interactions, which include not only ``encode'' and ``manipulate'' interactions but also ``introduce'' interactions (\texttt{annotate}, \texttt{import}, \texttt{derive}, \texttt{record}). We focus on ``encode'' and ``manipulate'' interactions from the typology because they are likely to be most familiar to Stack Overflow users, but we also mention coverage of ``introduce'' interactions in our analysis.

\vspace{-1.5mm}
\subsubsection{Stack Overflow Users Favor a Few Interaction Types.}
Our interaction breadth results are shown in \autoref{fig:interaction-types}.
We observed ``encode'' interactions, five of six ``manipulate'' interactions, and all four ``introduce'' interactions.
%Though all three interaction classes are observed, 
``Manipulate'' interactions (20.4\% of posts) were far more prevalent than ``encode'' (1.2\%) and ``introduce'' interactions (1.1\%). Given our results for visualization types, ``manipulate'' interactions are probably more popular and thus discussed more online. However, just two of the 11 interaction types (\texttt{select} and \texttt{navigate}) represent over 83\% of our observations.

We see some Stack Overflow users combining interactions in their interfaces. Here is one example, where a user aims to display specific statistics on hover \texttt{selection}s, while also supporting \texttt{filter}ing:
\vspace{-3mm}
\begin{quote}
    ``\textit{... I want my charts to have the total Overall Packages number (Object) available so I can display that in the tooltip, etc. This object will not change during the filter, I just need that total.}'' (post A-528)
    %\footnote{\raggedright\url{https://stackoverflow.com/questions/49038777/dc-js-how-to-provide-the-total-overall-column-value-using-group}}
\end{quote}
\vspace{-2.5mm}
However, Stack Overflow users tend to focus on one key interaction type in their code, often \texttt{select} or \texttt{navigate}.

\vspace{-1.5mm}
\subsection{Q6: Existing Support Structures for D3 May Mirror Rather than Enrich Users' Design Thinking}
\label{sec:usability:interaction-breadth}
\vspace{-1.5mm}

Given that Stack Overflow users seem to rely heavily on the D3 documentation, we analyze how the documentation relates to users' understanding of interactions, specifically through terminology.

\vspace{-1.5mm}
\subsubsection{Certain Terms are Associated with Specific Interaction Types.}
To better understand what terms are often used to describe interactions, we calculated the top five term roots that appear in Stack Overflow posts labeled with an interaction type.
For example, we see in \autoref{fig:interaction-types-topk} that ``zoom'', ``drag'', and ``pan'' are common descriptors for \texttt{navigation} interactions. ``Tooltips'' seem to be an important topic of discussion for \texttt{select} interactions.
In contrast, few terms seem to be associated with \texttt{filter} interactions, except for ``filter'' itself.

%We used GitHub's keyword search interface to identify issues that contain the top terms for the \texttt{select}, \texttt{navigate}, and \texttt{filter} interactions, such as ``zoom'' or ``filter''. The results are shown in \autoref{fig:interaction-types-issues}. We see that the relative frequencies of each term among GitHub issues are similar to what we observed on Stack Overflow. For example, issues that contain ``select'' represent over 10 percent of the total issues on GitHub (out of 2,048 total issues), and issues that contain ``zoom'' seem to be similarly significant. These results contrast with the findings of our visualization breadth analysis, where GitHub users seem to experiment with more sophisticated visualization types compared to Stack Overflow users. Our findings suggest that D3 users on both Stack Overflow and GitHub prioritize the same interaction types.

\begin{figure}
  \centering
  \includegraphics[width=0.7\columnwidth]{figures/interactionTypes_TopkPerCode.pdf}
  \vspace{-5mm}
  \caption{The top five term roots (x axis) counted across all coded posts (y axis) that mention an interaction type (color). Term root refers to the root of a word that appears in one or more posts.}
  \label{fig:interaction-types-topk}
  \vspace{-6mm}
\end{figure}


%\begin{figure*}
%  \begin{subfigure}[b]{0.2\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figures/interactionTypes.pdf}
%    \caption{Interactions: Coded Dataset.}
%    \label{fig:interaction-types}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.28\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figures/interactionTypes_issues.pdf}
%    \caption{Interactions: GitHub Issues.}
%    \label{fig:interaction-types-issues}
%  \end{subfigure}
%  %
%  \begin{subfigure}[b]{0.45\textwidth}
%    \centering
%    \includegraphics[width=\textwidth]{figures/interactionTypes_TopkPerCode.pdf}
%    \caption{Terms Per Interaction Type.}
%    \label{fig:interaction-types-topk}
%  \end{subfigure}
%  \vspace{-4mm}
%  \caption{(a) Total observations (y axis) for all interaction types from our taxonomy (x axis) in the qualitatively coded Stack Overflow data. (b) The total D3 issues on GitHub (y axis) that include the top two terms for \texttt{select}, \texttt{navigate}, and \texttt{filter} interactions (color, x axis). (c) The top five term roots (x axis) counted across all coded posts (y axis) that mention an interaction type (color). Term root refers to the root of a word that appears in one or more posts. \leilani{UPDATE}
%  %The most popular term roots are displayed on the x axis, term root frequency through bar height, and interaction types through color.
%  }
%  %\caption{Server setup results, displaying: response rate, or the fraction of all queries successfully answered within 100ms, and mean query duration calculated across all successfully answered queries. Results are faceted by dataset size (1M, 10M, or 100M rows) and type of data (flights, movies, or weather).}
%  \vspace{-4mm}
%\end{figure*}

\vspace{-1.5mm}
\subsubsection{Stack Overflow Users Describe Interaction Types With Different Levels of Specificity.}
We can also infer the granularity at which Stack Overflow users reason about specific interaction types by analyzing the specificity of the terms associated with each interaction type.
When we analyze \emph{how} interaction types are described, we see interesting differences in specificity. We observe fine-grained and detailed descriptions for the \texttt{select} interaction that showcase a variety of selection strategies. For example, ``hover,'' ``click,'' and ``drag'' are all used to describe the behavior of \texttt{select}.
Consider this description of a user's expected results for hover functionality across two maps:
\vspace{-2mm}
\begin{quote}
    ``\textit{... i have two maps (based on topojson-data, visualised through d3), and on mouseover over certain parts of map1, the corresponding parts of map2 should light up.}''(post A-280)
    %\footnote{\raggedright\url{https://stackoverflow.com/questions/30277374/moving-path-to-front-changes-selection}}
\end{quote}
\vspace{-2mm}
The user is describing specific JavaScript events relevant to the hover interaction (mouseover), and the expected result.

%``Zoom'' and ``drag'' are common descriptions of \texttt{navigation} interactions, but these descriptors are slightly higher-level than those for \texttt{select}. Consider the following description of a user's previous attempts at implementing a zoom interaction:
%\vspace{-2mm}
%\begin{quote}
%    ``\textit{Initially all the circles are in their correct positions. However when I click on the smaller circles, they shift position right before the zoom. When I click on the white circle to zoom back, you can see they are now permanently shifted. And when it does zoom, the circles don't zoom into the center of the viewport, like they do in the demo.}'' (PID 236)
%    %\footnote{\raggedright\url{https://stackoverflow.com/questions/28824577/d3-circles-shifting-position-on-click-to-zoom}}
%\end{quote}
%\vspace{-2mm}
%Here, we see both specific actions and self-referential definitions. For example, the user relies heavily on the word ``zoom'' to describe the behavior of the zoom interaction. At the same time, the user describes precise actions for manipulating specific marks, such as clicking on individual circles. It is possible that the user's understanding of the zoom interaction is clear in some ways but vague in others, leading to multiple levels of specificity in their post.

In contrast, \texttt{filter} interactions seem to be described primarily at a high level (e.g., using terms such as ``select'' or ``filter''), and are not often associated with particular low-level manipulations.
Consider the following quote from a user implementing a \texttt{filter} interaction:
\vspace{-2mm}
\begin{quote}
``\textit{Currently I have a script that is pulling data and filtering objects in a JSON file. I am trying to filter (show/hide) the restaurants by a star rating of 1-5.}'' (post C-251)
%\footnote{\raggedright\url{https://stackoverflow.com/questions/53617272/filtering-a-d3-js-map-using-jquery}}
\end{quote}
\vspace{-2mm}
Here, ``filter'' describes both the interaction and the intended behavior. Though the desired result is mentioned (i.e., showing or hiding restaurants), the manipulation to execute the filter (clicking on a checkbox) is not clearly specified. However, an embedded image does hint at checkboxes and restaurant rating stars being involved.

\vspace{-1.5mm}
\subsubsection{The Interactions in the D3 Documentation Match Observed Interactions on Stack Overflow.} To understand how the \textbf{D3 documentation} reflects the prevalence of certain interactions, we analyzed the the D3 API Reference. Three ``manipulate'' interactions seem to be well-represented in the documentation (with quoted topics in parentheses): \texttt{select} (``Search'', ``Brushes'', ``Selections''), \texttt{filter} (``Brushes'', ``selection.filter''), and \texttt{navigate} (``Dragging'', ``Zooming'').
Other interactions such as \texttt{change} have relevant topics (e.g., ``Time Formats''), but the documentation focuses on how to implement their functionality as immutable visualization components, rather than manipulable interaction widgets.

%\vspace{-1.5mm}
%\subsubsection{The D3 Documentation may be too Closely Tied to User Preferences.}
Stack Overflow users describe different interactions with varying levels of specificity, and the variations seem to be correlated with how these same interactions are described in the D3 documentation.
These results suggest that
%The varied specificity in how users describe interactions on Stack Overflow, paired with the varied specificity in how these same interactions are described in the D3 documentation, may suggest that 
Stack Overflow users may not understand these interaction types equally well.
On the one hand, the documentation could simply reflect the aspects of interactions that Stack Overflow users find confusing.
On the other hand, these findings could indicate that the D3 documentation may cause users to understand some interactions, or even parts of interactions, better than others. 
In either case, we believe these findings point to an interesting echo chamber between Stack Overflow and the D3 documentation.
%, and an evolving relationship between D3 users and D3 developers managed through the documentation.

\vspace{-1.5mm}
\subsection{Takeaways for Interaction Breadth Analysis}
\vspace{-1.5mm}

Not all users describe their challenges on Stack Overflow with the same quality and specificity~\cite{ravi2014great}. However, we do see some general trends.
In response to \textbf{Q6}, Stack Overflow users seem to favor a narrow subset of interaction types. Specifically, we observe only five of seven ``manipulate'' interactions and one out of four ``introduce'' interactions from our taxonomy. Subsequent analyses of the D3 documentation reveal that these interaction types are not described equally well (if at all), suggesting that some interaction types are not prioritized among Stack Overflow users.
Given that observations on Stack Overflow seem to correlate with the popularity of visualizations rather than confusion around particular visualizations (see \autoref{sec:usability:visualization-breadth}), we hypothesize that these gaps reflect a lack of user awareness or interest in implementing certain visualization and interaction types.
Our results suggest that the non-uniform coverage of interaction types in the D3 documentation, both in terms of occurrence and specificity, may reflect users' \emph{understanding} of different interaction types, and thus how clearly Stack Overflow users can articulate challenges encountered when implementing these interactions. Taking this idea one step further, the D3 documentation could potentially be a driver of this skew in user preferences, leading to visualization design bias among Stack Overflow users. However correlation does not equal causation; we leave quantitative evaluation of these new hypotheses for future work.
